HD 119130 b is not an "ultra-dense" sub-Neptune

We present a revised mass measurement for HD 119130 b (aka K2-292 b), a transiting planet ($P = 17$ days, $R_\mathrm{p} = 2.63^{+0.11}_{-0.10}$ $R_\mathrm{\oplus}$) orbiting a chromospherically inactive G dwarf, previously thought to be one of the densest sub-Neptunes known. Our follow-up Doppler observations with HARPS, HARPS-N, and HIRES reveal that HD 119130 b is, in fact, nearly one-third as massive as originally suggested by its initial confirmation paper. Our revised analysis finds $M_\mathrm{p} = 8.8 \pm 3.2$ $M_\mathrm{\oplus}$ ($M_\mathrm{p} < 15.4$ $M_\mathrm{\oplus}$ at 98\% confidence) compared to the previously reported $M_\mathrm{p} = 24.5 \pm 4.4$ $M_\mathrm{\oplus}$. While the true cause of the original mass measurement's inaccuracy remains uncertain, we present the plausible explanation that the planet's radial velocity (RV) semi-amplitude was inflated due to constructive interference with a second, untreated sinusoidal signal in the data (possibly rotational modulation from the star). HD 119130 b illustrates the complexities of interpreting the RV orbits of small transiting planets. While RV mass measurements of such planets may be precise, they are not necessarily guaranteed to be accurate. This system serves as a cautionary tale as observers and theorists alike look to the exoplanet mass-radius diagram for insights into the physics of small planet formation.

==> systemproperties.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%% HD 119130. System I %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Values from Luque et al. (2019) that are adopted by us
\newcommand{\logrhkI}{$-5.08 \pm 0.05$\xspace}
\newcommand{\mstarILXIX}{$1.00 \pm 0.03$\xspace}
\newcommand{\rstarILXIX}{$1.09 \pm 0.03$\xspace}
\newcommand{\periodIbLXIX}{$16.9841 \pm 0.0008$\xspace}
\newcommand{\tcIbLXIX}{$2458180.2842^{+0.0017}_{-0.0015}$\xspace}
\newcommand{\rpIb}{$2.63^{+0.11}_{-0.10}$\xspace}

\newcommand{\periodIb}{$16.9841 \pm 0.0008$\xspace}
\newcommand{\tcIb}{$2460232.8 \pm 0.9$\xspace}
\newcommand{\KIb}{$2.2 \pm 0.8$\xspace}
\newcommand{\mpIb}{$8.8 \pm 3.2$\xspace}
\newcommand{\mpIbupperlim}{$15.4$\xspace} % 98% confidence
\newcommand{\rhoIb}{$2.7 \pm 1.0$\xspace}
\newcommand{\periodIc}{$200.3 \pm 2.9$\xspace}
\newcommand{\tcIc}{$2460111.9 \pm 6.9$\xspace}
\newcommand{\KIc}{$4.9 \pm 1.2$\xspace}
\newcommand{\msiniIc}{$44.4 \pm 10.9$\xspace}

% Values from Luque et al. (2019) used for comparison
\newcommand{\mpIbLXIX}{$24.5 \pm 4.4$\xspace} % Mass measurement from Luque et al. (2019)
\newcommand{\rhoIbLXIX}{$7.4^{+1.6}_{-1.5}$\xspace} % Density from Luque et al. (2019)

\newcommand{\gammarvCARMENESI}{$-0.3 \pm 3.2$\xspace}
\newcommand{\sigmarvCARMENESI}{$4.8 \pm 1.4$\xspace}
\newcommand{\gammarvHARPSI}{$-0.7 \pm 1.0$\xspace}
\newcommand{\sigmarvHARPSI}{$2.7 \pm 0.8$\xspace}
\newcommand{\gammarvHARPSNI}{$1.4 \pm 1.0$\xspace}
\newcommand{\sigmarvHARPSNI}{$2.8 \pm 1.1$\xspace}
\newcommand{\gammarvHIRESI}{$-1.7 \pm 1.2$\xspace}
\newcommand{\sigmarvHIRESI}{$1.7 \pm 1.0$\xspace}

